Theory and Design of Super-resolution Haptic Skins

Haptic feedback is important to make robots more dexterous and effective in unstructured environments. High-resolution haptic sensors are still not widely available, and their application is often bound by the resolution-robustness dilemma. A route towards high-resolution and robust skin embeds a few sensor units (taxels) into a flexible surface material and uses signal processing to achieve sensing with super-resolution accuracy. We propose a theory for geometric super-resolution to guide the development of haptic sensors of this kind and link it to machine learning techniques for signal processing. This theory is based on sensor isolines and allows us to predict force sensitivity and accuracy in contact position and force magnitude as a spatial quantity. We evaluate the influence of different factors, such as elastic properties of the material, structure design, and transduction methods, using finite element simulations and by implementing real sensors. We empirically determine sensor isolines and validate the theory in two custom-built sensors with barometric units for 1D and 2D measurement surfaces. Using machine learning methods for the inference of contact information, our sensors obtain an unparalleled average super-resolution factor of over 100 and 1200, respectively. Our theory can guide future haptic sensor designs and inform various design choices.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
